S2 Reducer: High-Performance Sparse Communication to Accelerate Distributed Deep Learning

Distributed stochastic gradient descent (SGD) approach has been widely used in large-scale deep learning, and the gradient collective method is vital to ensure the training scalability of the distributed deep learning system. Collective communication such as AllReduce has been widely adopted for the distributed SGD process to reduce the communication time. However, AllReduce incurs large bandwidth resources while most gradients are sparse in many cases since many gradient values are zeros and should be efficiently compressed for bandwidth saving. To reduce the sparse gradient communication overhead, we propose Sparse-Sketch Reducer (S2 Reducer), a novel sketch-based sparse gradient aggregation method with convergence guarantees. S2 Reducer reduces the communication cost by only compressing the non-zero gradients with count-sketch and bitmap, and enables the efficient AllReduce operators for parallel SGD training. We perform extensive evaluation against four state-of-the-art methods over five training models. Our results show that S2 Reducer converges to the same accuracy, reduces 81\% sparse communication overhead, and achieves 1.8$ \times $ speedup compared to state-of-the-art approaches.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> section/analysis.tex <==
\section{Theoretical Analysis}
In this section, we first quantify the variance bound of CASQ. This bound indicates that CASQ can converge in a single node, then we prove its convergence in a distributed setting.

\subsection{Variance Bound of CASQ}
%cluster influence, routine; symbol definition; expectation and variance without assumption 
In Theorem~\ref{theo:casloss}, we firstly quantify the expectation and variance of the compression error based on the random mapping of each gradient and prove that the variance is inversely proportional to the number of elements in its mapped bucket. Then, we bound the variance and the second moment of the estimated gradient vector with $\|g\|^2_2$. %The full proof is deferred to Appendix~\ref{appen:theo2}.

%expectstion and variance in assumptipn;
\begin{theorem}\label{theo:casloss}
    Let $\left\{g_j^i\right\} $ denote the gradients inserted to the bucket corresponding to the $ j^{th} $ gradient. Let $ n_j=\left|\left\{g_j^i\right\}\right| $ denote the number of item inserted to the bucket corresponding to the $ j^{th} $ gradient. Suppose that $ j $ belongs to cluster $k$, where gradients are i.i.d with expectation $\mu_k$ and variance $\sigma _k$, let $ N_k $ denotes the number of elements in $ k $. Then we have the following:
    \begin{enumerate}
        \item $ \mathbb{E} \left[\hat{g}(j) - g(j) \right] =\left(1-\frac{m}{N_k}\right)\left(\mu_k-g(j)\right) $,
        \item $ Var\left[\hat{g}(j)-g(j)\right] =\frac{m(N_k-1)}{{N_k}^{2}} \left(\delta_k^{2}+\left(1-\frac{1}{m}\right) \mu_k^{2}\right) $,
        \item $ \mathbb{E}\left[\|\hat{g}\|_{2}^{2}\right]\leq \|g\|_{2}^{2} $,
        \item{\label{theo:caslossbound}} $ \mathbb{E}\left[\|\hat{g}-g\|_{2}^{2}\right]  \leq(1-\delta){\left\|g\right\|}^2$ for $\delta \in (0,1)$ if $m \ll N_k$ holds.
    \end{enumerate} 
    %   (a) $ \mathbb{E} \left[\hat{g}(j) - g(j) \right] = {(n_j-1)\left(\mu_k-g(j)\right)}/{n_j}$, (b) $ Var\left[\hat{g}(j)-g(j)\right] =({N_k-1}) \left(\sigma_k^2+(1-{1}/{m})\mu_k^2\right)/{n_j^2}m$, (c)  $ \mathbb{E}\left[\|\hat{g}\|_{2}^{2}\right]\leq \|g\|_{2}^{2} $, (d) $ \mathbb{E}\left[\|\hat{g}-g\|_{2}^{2}\right]  \leq(1-\delta){\left\|g\right\|}^2$ for $\delta \in (0,1)$ if $m \ll N_k$.
\end{theorem} 
\begin{IEEEproof}
    The error of a sketch can be quantified as $\hat{g}-g=A A^{T} g-g=\left(A A^{T}-I\right) g$, where $I$ denotes the identity matrix. $AA^T$ is a $N\times N$ symmetric matrix, where each entry $(i, j)$ is one when the $i^{th}$ and $j^{th}$ gradients mapped into the same bucket, {i.e.}: $A(i, :)=A(j, :)$, and zero otherwise. It means that the diagonal entries are all set to ones.  Each gradients is mapped according to a uniformly-random hash function, so that $Pr[AA^T(i, j)=1]=\frac{1}{m}$ and $Pr[AA^T(i, j)=1]=1-\frac{1}{m}$, which follows Bernoulli distribution. 
    
    Let $\Phi=AA^T-I$, then each non-diagonal entry in $\Phi$ is the same as that in $AA^T$,  we have $\Phi_{i\neq j}(i, j)\sim Bernoulli(\frac{1}{m})$, and the diagonal entries are zeros, which means $\mathbb{E}[\Phi_{i\neq j}(i, j)]=\frac{1}{m}$ and $Var[\Phi_{i\neq j}(i, j)]=\frac{1}{m}\cdot(1-\frac{1}{m})]$.
    
    Note that a gradient is randomly mapped to the buckets, then $ n_j  $ is viewed as a constant $ \frac{N_k}{m} $. The approximated $g(j)$ is the averaged bucket value, so that the expectation of loss is: 
    \begin{align*}
        \mathbb{E}[\hat{g}(j)-g(j)]=&\mathbb{E}\left[\frac{{\sum{g_j^i}}}{n_j}-g(j)\right]\\
        =&\frac{1}{n_j}\mathbb{E}\left[\sum_{i=1}^{n_j-1}\left({g_j^i - g(j)}\right)\right]\\
        =&\frac{(n_j-1)\left(\mu_k-g(j)\right)}{n_j}\\
        =&\left(1-\frac{m}{N_k}\right)\left(\mu_k-g(j)\right)\\
        \leq&\frac{(N-1) \mu}{m}
    \end{align*}
    
    Recall that we derive the gradients from Equation~\ref{eq:esti_grad_cluster}, which has the similar structure form with $AA^Tg$ for each cluster, and the random variable in one cluster is independent of that in other clusters. Therefore, we note the variance of $\hat{g}(j)-g(j)$ as below:   
    \begin{align*}
        & {Var}\left[\hat{g}(j)-g{(j)}\right] \\
        =& {Var}\left[\sum_{i=1}^{N_k}\left(A\left(A^{T} A\right)^{-1} A^{T}\right)(i, j) g{(i)}- g(j)\right] \\
        =&{Var}\left[\frac{\sum_{i=1}^{N_k}\left(A A^{T}\right)(i, j) g{(i)}}{n_{j}}- g(j)\right]\\ 
        =&\frac{1}{n_{j}^{2}} {Var}\left[\sum_{i=1}^{N_k}\left(A A^{T}\right)(i, j) g{(i)}-n_{j} {g}{(j)}\right]\\
        =&\frac{1}{n_{j}^{2}} {Var}\left[\sum_{i=1}^{N_k-1} \Phi\left(i, j\right) g(i)-(n_{j} -1)g{(j)}\right]\\
        =&\frac{N_k-1}{n_{j}^{2}}  {{Var}[\Phi(i, j) g(i)]} \\
        =&\frac{N_k-1}{n_{j}^{2}}\cdot \frac{1}{m}\left(\delta_k^{2}+\left(1-\frac{1}{m}\right) \mu_k^{2}\right)\\
        =&\frac{m(N_k-1)}{{N_k}^{2}} \left(\delta_k^{2}+\left(1-\frac{1}{m}\right) \mu_k^{2}\right)\\
        %\leq&\frac{N-1}{m}\left(\sigma^{2}+\left(1-\frac{1}{m}\right) \mu^{2}\right)
    \end{align*}
    
    % For a specific $j$, $g(j)$ is constant when other gradients in its bucket vary, so we have $Var\left[\hat{g}(j)\right]=Var\left[\hat{g}(j)-g{(j)}\right]$. 
    
    To prove the bound of $\mathbb{E}\left[\left\|\hat{g} \right\|^2_2\right]$, we note the following:
    \begin{align*}  
        \mathbb{E}\left[{\hat{g}{(j)}}^{2}\right] &=\mathbb{E}\left[\left(\frac{\sum_{i=1}^{n_j} g_{j}^{i}}{n_{j}}\right)^{2}\right] \\
        & \leq \mathbb{E}\left[\frac{\sum_{i=1}^{n_j} \left(g_{j}^{i}\right)^{2}}{n_{j}}\right]
    \end{align*}
    
    Where the second line follows the fact that the arithmetic mean is less or equal than the quadratic mean. Hence, we have
    \begin{align*}
        \mathbb{E}\left[\|\hat{g}\|_{2}^{2}\right] &=\sum_{j=1}^{N} \mathbb{E}\left[\left(\hat{g}{(j)}\right)^2\right] \\
        &=\sum^{K}_{k=1} \sum_{j=1}^{N_k} \mathbb{E}\left[\left(\frac{\sum_{i=1}^{n_j} g_{j}^{i}}{n_{j}}\right)^{2}\right]\\
        &\leq\sum_{k=1}^{K} \sum_{j=1}^{N_{k}} \mathbb{E}\left[\frac{\sum_{i=1}^{n_j} \left(g_{j}^{i}\right)^{2}}{n_{j}}\right]\\
        &=\sum_{k=1}^{K} \sum_{j=1}^{N_{k}} g(j)^{2}\\
        &=\|g\|_{2}^{2}
    \end{align*}
    
    Based on the lemma above, we prove the bound of $\mathbb{E}\left[{\left\|{\hat{g}-g}\right\|}_2^2\right]$ as follows:
    
    \begin{align*}
        &\mathbb{E}\left[\|\hat{g}-g\|_{2}^{2}\right] =\sum^{K}_{k=1} \sum_{j=1}^{N_k} \mathbb{E}\left[\left(\hat{g}{(j)}-g(j)\right)^2\right] \\
        =&\sum^{K}_{k=1} \sum_{j=1}^{N_k}Var\left[\hat{g}{(j)}-g(j)\right]+\mathbb{E}\left[\hat{g}{(j)}-g(j)\right]^2\\
        =&\sum^{K}_{k=1} \sum_{j=1}^{N_k}\frac{N_k-1}{n_{j}^{2}}\cdot \frac{1}{m}\left(\delta_k^{2}+\left(1-\frac{1}{m}\right) \mu_k^{2}\right)\\
        &+{\left(\frac{(n_j-1)\left(\mu_k-g(j)\right)}{n_j}\right)}^2\\
        \leq&\sum^{K}_{k=1} \sum_{j=1}^{N_k}\frac{N_k}{n_{j}^{2}}\cdot \frac{1}{m}\left(\delta_k^{2}+\left(1-\frac{1}{m}\right) \mu_k^{2}\right)+{\left(\mu_k-g(j)\right)}^2\\
        =&\sum^{K}_{k=1} \sum_{j=1}^{N_k}\frac{m}{N_k}\left(\delta_k^{2}+\left(1-\frac{1}{m}\right) \mu_k^{2}\right)+{\mu_k^2-2\mu_kg(j)+{g(j)}^2}\\
        =&\sum^{K}_{k=1} {m}\left(\delta_k^{2}+\left(1-\frac{1}{m}\right) \mu_k^{2}\right)+N_k\mu_k^2-2\mu_k{\left\|g_k\right\|}_1+{\left\|g_k\right\|}_2^2\\
        \overset{a}{\approx}&\sum^{K}_{k=1} \mu_k\left(N_k\mu_k-2{\left\|g_k\right\|}_1\right)+{\left\|g_k\right\|}_2^2\\
        \leq&\sum^{K}_{k=1} {\left\|g_k\right\|}_2^2={\left\|g\right\|}_2^2
        %       =&\sum^{K}_{k=1} \sum_{j=1}^{N_k} \mathbb{E}\left[\left(\frac{\sum_{i=1}^{n_j} g_{j}^{i}}{n_{j}}- g(j)\right)^{2}\right]\\
        %       =&\sum^{K}_{k=1} \sum_{j=1}^{N_k} \mathbb{E}\left[\frac{1}{n_{j}^2}\left(\sum_{i=1}^{n_j-1}\left(g_{j}^{i}- g(j)\right)\right)^{2}\right]\\
        %       \leq &\sum_{k=1}^{K} \sum_{j=1}^{N_{k}} \mathbb{E}\left[\frac{n_j-1}{n_{j}^2}\sum_{i=1}^{n_j-1}\left(g_{j}^{i}- g(j)\right)^{2}\right]\\
        %       \leq &\sum_{k=1}^{K} \sum_{j=1}^{N_{k}} \mathbb{E}\left[\frac{{(n_j-1)}^2}{n_{j}^2}\sum_{i=1}^{n_j-1}\left({(g_{j}^{i})}^2+ {g(j)}^2\right)\right]\\
        %       \leq &\sum_{k=1}^{K} \sum_{j=1}^{N_{k}} \mathbb{E}\left[\frac{n_j-1}{n_{j}^2}\left(\sum_{i=1}^{n_j}{(g_{j}^{i})}^2+{n_j}{g(j)}^2\right)\right]\\
        %       =&\sum_{k=1}^{K} \sum_{j=1}^{N_{k}} \mathbb{E}\left[\sum_{i=1}^{n_j}\frac{2}{n_{j}^2}{(g_{j}^{i})}^2\right] +\mathbb{E}\left[\frac{2}{n_{j}}\right]{g(j)}^2\\
        %       =&\sum_{k=1}^{K} \sum_{j=1}^{N_{k}} \frac{2m}{N_k}\left(\mathbb{E}\left[{(g_{j}^{i})}^2\right] +{g(j)}^2\right)\\
        %       \leq &\sum_{k=1}^{K} \frac{4m}{N_k}{\left\|g_k\right\|}^2 \leq(1-\delta){\left\|g\right\|}^2
    \end{align*}
    
    Where {(a)} follows from the setting of sketch that $ m\ll N_k $. As a result, we have $\mathbb{E}\left[\|\hat{g}-g\|_{2}^{2}\right]\leq (1-\delta){\left\|g\right\|}^2$ for $\delta \in (0,1)$, as claimed.
    
\end{IEEEproof}
%Accordingly, we dramatically decline the quantization loss compared with CM-based approach and bound the variance. 

%Theorem~\ref{theo:casloss} implies that the hyperparameter $ m $ controls the precision and variance of estimation: the queried gradients are getting closer to the original values when setting a larger $ m $, but it expanding the variance in the meantime. We take a trade-off between the precision and variance by calculating $ m $ adaptively in Section~\ref{subsec:merge}.

%A remaining problem is that the expectation of approximated value is not the unbiased estimation of the original $g(j)$ or $\bar{g}(j)$ even now, which is a prerequisite of stochastic gradients. However, based on the connection among variable distributions of similar stochastic gradients noted in Section~\ref{subsec:cluster}, we can deduce that the average value in a cluster is an unbiased estimation of $\bar{g}(j)$, and can also bound the range of estimated gradients. 
%%probability of bigger than a value
%
%\begin{theorem}{\label{theo:unbias}}
%   Let $\left\{g_j^i\right\} $ and $ n_j$ are defined as that in Theorem~\ref{theo:casloss}.   Let $M$ denote the bound such that $ \forall{g{_j^i}}, \left|g{_j^i}-\bar{g}(j)\right| \leq M $.
%   Suppose that the stochastic gradients in one cluster have an identical distribution $\mathcal{D}_2$, which is empirically observed in experiments. If gradients maintain the same cluster assignment among distributed nodes, we have the following results:
%   \begin{enumerate}
%       \item The estimated value $\hat{g}(j)$ is an unbiased estimation of $\bar{g}(j)$.
%       \item The range of estimated gradients is bounded with probability ${Pr}\left(\left|\hat{g}{(j)}-\bar{g}(j)\right| \geq a\right) \leq \frac{M^{2}}{a^{2} {n_{j}}^{2}}$. Furthermore, we have $ {Pr}\left(\left|\hat{g}{(j)}-g{_j^i}\right| \geq a\right) \leq \frac{M^{2}}{(a-M)^{2} {n_{j}}^{2}} $
%   \end{enumerate}
%\end{theorem}

\subsection{Convergence of CASQ}
 %The detailed proof is stated in Appendix~\ref{appen:CAS-SGD}.
The variance bound of CASQ in Theorem~\ref{theo:casloss} immediately implies that CASQ quantization is a $\delta$-approximate compressor~\cite{karimireddy2019error}. Then we can prove the convergence of CASQ in a single node with this property and extend the result to distributed CASQ based on Lemma~\ref{lem:error} and~\ref{lem:declinevalue}. The analysis shows that the CASQ converges at a rate matching that of vanilla distributed SGD under standard assumptions of smoothness of the loss function and the variance of gradients.

\begin{assumption}{\label{assum:cas-sgd}}
    In distributed setting with $ W $ worker nodes, let function $ f: \mathbb{R}^d \rightarrow \mathbb{R}$ is L-smooth, and for any $ \boldsymbol{\omega} \in \mathbb{R}^d $, both the local and global gradients are bounded, i.e.: $\exists \sigma_{i}, \sigma \in \mathbb{R} $ such that $ \left\|\nabla f_{i}({\boldsymbol{\omega}})\right\| \leq \sigma_{i},\|\nabla f(\boldsymbol{\omega})\| \leq \sigma $.
\end{assumption}

\begin{definition}[$\delta$-approximate compressor]{\label{def:comp}}
    An operator $\mathcal{C}(\cdot):  \mathbb{R}^d \rightarrow \mathbb{R}^d $ is a $ \delta $-approximate compressor if $\exists \delta \in (0, 1] $ such that 
    
    $\left\| \mathcal{C}(\boldsymbol{\omega}) - \boldsymbol{\omega} \right\|^2_2 \leq  \left(1-\delta\right)\left\|\boldsymbol{\omega}\right\|^2_2 $, $\forall \boldsymbol{\omega} \in \mathbb{R}^d $.
\end{definition}


    
\begin{lemma}{\label{lem:error}}
    Under the Assumption~\ref{assum:cas-sgd}, the error compensation $ e_t^i $ in worker node $ i $ is bounded for all iteration $ t $ in CASQ:
    \begin{equation*}
        \left\|{e}_t^i \right\|^{2} \leq \frac{4(1-\delta)}{\delta^{2}} \sigma_{i}^{2}
    \end{equation*}  
\end{lemma}






\begin{IEEEproof}
    As shown in the Definition \ref{def:comp}, $\mathcal{C}(\cdot)$ is a $\delta$-approximate compressor. Combined with the definition of the error sequence, we have
    \begin{align*}
            \left\|{e}_{t+1}^{i}\right\|_{2}^{2}=&\left\|{g}_{t}^{i}-\mathcal{C}({g}_{t}^{i})\right\|_{2}^{2}\leq(1-\delta)\|{g}_{t}^{i}\|_{2}^{2}\\
            =&(1-\delta)\|\nabla f_{i}({\omega}_{t})+{e}_{t}^{i}\|_{2}^{2}\\
            \le& (1-\delta)\big[(1+\gamma)\|{e}_{t}^{i}\|_{2}^{2}+(1+1/\gamma)\|\nabla f_{i}({\omega}_{t})\|_{2}^{2}\big],
    \end{align*}
    where we used the Young's inequality (for any $\gamma>0$). Noticed that ${e}_{0}^{i}=0$ and $\nabla f_{i}({\omega}_{t})$ is bounded in Assumption \ref{assum:cas-sgd}, simple computation yields
    \begin{align*}
        \begin{split}
            &\left\|{e}_{t+1}^{i}\right\|_{2}^{2}\\
            \le& (1-\delta)(1+\gamma)\|{e}_{t}^{i}\|_{2}^{2}+(1-\delta)(1+1/\gamma)\|\nabla f_{i}({\omega}_{t})\|_{2}^{2}\\
            \le&(1-\delta)(1+\gamma)^{t+1}\|{e}_{0}^{i}\|_{2}^{2}\\
            &+\sum_{k=0}^{t}\big[(1-\delta)(1+\gamma)\big]^{t-k}(1-\delta)(1+1/\gamma)\|\nabla f_{i}({\omega}_{t})\|_{2}^{2}\\
             \le& \sum_{k=0}^{\infty}\big[(1-\delta)(1+\gamma)\big]^{t-k}(1-\delta)(1+1/\gamma) \sigma_{i}^{2}\\
            =&\frac{(1-\delta)(1+1 / \gamma)}{1-(1-\delta)(1+\gamma)} \sigma_{i}^{2}.
        \end{split}
    \end{align*}
    Let us pick $\gamma=\frac{\delta}{2(1-\delta)}$ such that $1+1/\gamma=(2-\delta)/\delta \leq 2/\delta$. Then we have
    \begin{align*}
        \left\|{e}_{t+1}^{i}\right\|_{2}^{2}\le\frac{2(1-\delta)(1+1 / \gamma)}{\delta} \sigma_{i}^{2} \leq \frac{4(1-\delta)}{\delta^{2}} \sigma_{i}^{2}.
    \end{align*}
    
\end{IEEEproof}


\begin{lemma}{\label{lem:declinevalue}}
    Under the Assumption~\ref{assum:cas-sgd}, given the learning rate $ 0<\eta<2/(\rho+L) $, $ \rho>0 $, the loss function satisfies:
    
    \begin{equation*}
        f\left(\boldsymbol{\nu}_{t+1}\right)-f\left(\boldsymbol{\nu}_{t}\right) \leq \Delta_{CAS}^{t}  
    \end{equation*}
    
    Where $ \boldsymbol{\nu}_{t}:=\boldsymbol{\omega}_{t}-\eta \cdot \sum_{i=1}^{W} {e}_t^i $ and
    
    \begin{align*}
        \Delta_{CAS}^{t}:=&-\eta\left(1-\frac{(\rho+L) \eta}{2}\right)\left\|\nabla f\left(\boldsymbol{\omega}_{t}\right)\right\|^{2}\\
        +&\frac{L^{2} \eta^{2}}{2 \rho}\left\|\sum_{i=1}^{W} {e}_t^i\right\|^{2}    
    \end{align*}
    
\end{lemma}

\begin{IEEEproof}
    From the definition of the sequence $\{{\nu}_{t}\}_{t=0,1,\cdots}$, we have that
    \begin{align*}
        \begin{split}
            {\nu}_{t+1}&={\omega}_{t+1}-\eta  \sum_{i=1}^{W}\mathbf{e}_{t+1}^{i}\\
            &={\omega}_{t}-\eta \sum_{i=1}^{W}\mathcal{C}({g}_{t}^{i})-\eta  \sum_{i=1}^{W}\mathbf{e}_{t+1}^{i}\\
            &={\omega}_{t}-\eta \sum_{i=1}^{W}{g}_{t}^{i}\\
            &={\omega}_{t}-\eta \sum_{i=1}^{W}\mathbf{e}_{t}^{i}-\eta \sum_{i=1}^{W}\nabla f_{i}({\omega}_{t})\\
            &={\nu}_{t}-\eta \nabla f({\omega}_{t}).
        \end{split}
    \end{align*}
    Since the function $f$ is $L$-smooth, i.e.
    \begin{align*}
        \begin{split}
            &\|\nabla f(\mathbf{x})-\nabla f(\mathbf{y})\|_{2} \leq L\|\mathbf{x}-\mathbf{y}\|_{2},\\
            f(\mathbf{x})&- f(\mathbf{y}) \leq \langle \nabla f(\mathbf{y}), \mathbf{x} - \mathbf{y} \rangle +\frac{L}{2}\| \mathbf{x} - \mathbf{y} \|_{2}^{2}.
        \end{split}
    \end{align*}
    We have
    
    \begin{equation}
        \label{eqn_39}
        \begin{split}
            &f({\nu}_{t+1})-f({\nu}_{t}) \leq \langle \nabla f({\nu}_{t}), {\nu}_{t+1}-{\nu}_{t} \rangle +\frac{L}{2}\|{\nu}_{t+1}-{\nu}_{t}\|_{2}^{2}\\
            \leq& \langle \nabla f({\omega}_{t}), {\nu}_{t+1}-{\nu}_{t} \rangle + \langle \nabla f({\nu}_{t})-f({\omega}_{t}), {\nu}_{t+1}-{\nu}_{t} \rangle\\
            &+\frac{L}{2}\|{\nu}_{t+1}-{\nu}_{t}\|_{2}^{2}\\
            \leq& -\eta(1-\frac{L\eta}{2})\|\nabla f({\omega}_{t})\|_{2}^{2}+\frac{\rho}{2}\|{\nu}_{t+1}-{\nu}_{t}\|_{2}^{2}\\
            &+\frac{1}{2\rho}\| \nabla f({\nu}_{t})-f({\omega}_{t})\|_{2}^{2}\\
            \leq& -\eta \big(1-\frac{(L+\rho)\eta}{2}\big)\|\nabla f({\omega}_{t})\|_{2}^{2}+\frac{L^{2}}{2\rho}\|{\nu}_{t}-{\omega}_{t}\|_{2}^{2}\\
            \leq& -\eta\big(1-\frac{(\rho+L)\eta}{2}\big)\left\|\nabla f({\omega}_{t})\right\|_{2}^{2}+\frac{L^{2} \eta^{2}}{2 \rho}\Big\|\sum_{i=1}^{W}\mathbf{e}^{i}_{t}\Big\|_{2}^{2}.
        \end{split}
    \end{equation}
    The third inequality follows from the mean-value inequality and holds for any $\rho>0$.
    
\end{IEEEproof}

%The Proof of Lemma~\ref{lem:error} and~\ref{lem:declinevalue} are stated in Appendix.

\begin{theorem}[Non-convex convergence of CASQ]{\label{thm:CAS-SGD}}
    Given $0<\rho$, $ 0<\eta<2/(\rho+L)$, the CASQ outputs model parameters $ \{\boldsymbol{\omega}_t \}_{t\geq0}$ in $ T $ iterations. Under the Assumption~\ref{assum:cas-sgd},
    \begin{equation*}
        \min _{0 \leq t \leq T}\left\|\nabla f\left(\boldsymbol{\omega}_{t}\right)\right\|^{2} \leq \frac{a\left(f^{0}-f^{*}\right)}{\eta \cdot(T+1)}+b \cdot \eta
    \end{equation*}
    Where $ f_{0}:=f\left(\boldsymbol{\omega}_{0}\right)$, $f^{*}$ is the optimal solution, $ a:=\frac{2}{(2-(\rho+L) \eta)}$, $ b:=\frac{4 L^{2} W \sigma^{2}(1-\delta)}{\rho \delta^{2}(2-(\rho+L) \eta)}  $ and $ \sigma^{2}:=\sum_{i=1}^{W} \sigma_{i^{\circ}}^{2} $
\end{theorem}

\begin{IEEEproof}
    The one-step descent of CASQ is given in Lemma \ref{lem:declinevalue}, and the residual error is bounded in Lemma \ref{lem:error}. Summing the terms in (\ref{eqn_39}) over $t$ gives
    \begin{equation}
        \label{eqn_40}
        \begin{split}
        f({\nu}_{T+1})-f({\nu}_{0}) &\leq -\eta\big(1-\frac{(\rho+L)\eta}{2}\big)\sum_{t=0}^{T}\left\|\nabla f({\omega}_{t})\right\|_{2}^{2}\\
        &+\frac{2L^{2} \eta^{2}(1-\delta)}{\rho \delta^{2}}(T+1)W \sigma^{2},
        \end{split}
    \end{equation}
    where we used
    \begin{align*}
        \nonumber
        \|\sum_{i=1}^{W}\mathbf{e}_{t}^{i}\|_{2}^{2} &\leq W \sum_{i=1}^{W}\|\mathbf{e}_{t}^{i}\|_{2}^{2} \\
        &\leq W\cdot \frac{4(1-\delta)}{\delta^{2}} \sum_{i=1}^{W}\sigma_{i}^{2}:=\frac{4(1-\delta)}{\delta^{2}} W\sigma^{2},
    \end{align*}
    where $\sigma^{2}:=\sum_{i=1}^{W}\sigma_{i}^{2}$.
    
    Noticed that ${\nu}_{0}={\omega}_{0}$ and $f^{*}$ is the optimal value. Given step-size $\eta<2/(\rho+L)$, rearranging the terms in (\ref{eqn_40}) and averaging over $t$ lead to
    \begin{align*}
        \nonumber
        \begin{split}
            &\frac{1}{T+1}\sum_{t=0}^{T}\left\|\nabla f({\omega}_{t})\right\|_{2}^{2} \\
            \leq& \frac{f({\nu}_{0})-f({\nu}_{T+1})}{\eta(T+1)\big(1-\frac{(\rho+L)\eta}{2}\big)}+\frac{2L^{2} \eta(1-\delta)W \sigma^{2}}{\rho \delta^{2}\big(1-\frac{(\rho+L)\eta}{2}\big)}\\
             \leq& \frac{2(f^{0}-f^{*})}{\eta(T+1)\big(2-(\rho+L)\eta\big)}+\frac{4L^{2} \eta(1-\delta)W \sigma^{2}}{\rho \delta^{2}\big(2-(\rho+L)\eta\big)}
        \end{split}
    \end{align*}
    Then we finished this proof.
    
\end{IEEEproof}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
    \renewcommand{\arraystretch}{1.4}
    \centering
    \caption{Validation accuracy on CIFAR-10/100 using 2/3-bit quantization (except for SuperSGD and TernGrad) with 4-GPUs.}
    \label{tab:test_acc}
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|}
        \hline
        &
        \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}ResNet32\\ CIFAR-10\end{tabular}} &
        \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}ResNet32\\ CIFAR-100\end{tabular}} &
        \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}ResNet56\\ CIFAR-100\end{tabular}} &
        \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}ResNet110\\ CIFAR-100\end{tabular}} \\ \hline
        Methods  & 2-bit                & 3-bit               & 2-bit           & 3-bit           & 2-bit           & 3-bit           & 2-bit           & 3-bit           \\ \hline \hline
        D-SGD & \multicolumn{2}{c|}{\bfseries{92.61$\pm$0.05}} & \multicolumn{2}{c|}{\bfseries{67.39$\pm$0.06}} & \multicolumn{2}{c|}{\bfseries{69.36$\pm$0.06}} & \multicolumn{2}{c|}{\bfseries{71.52$\pm$0.13}} \\ \hline
        Qinf     & 87,14$\pm$0.03        & 89.90$\pm$0.02       & 60.32$\pm$0.08   & 64.22$\pm$0.14   & 62.81$\pm$0.06   & 66.45$\pm$0.06   & 63.29$\pm$0.12   & 67.75$\pm$0.08   \\ \hline
        TernGrad & \multicolumn{2}{c|}{89.78$\pm$0.09}          & \multicolumn{2}{c|}{64.19$\pm$0.08} & \multicolumn{2}{c|}{65.35$\pm$0.06} & \multicolumn{2}{c|}{66.13$\pm$0.14} \\ \hline
        NUQSGD   & 65.19$\pm$0.05        & 82.36$\pm$0.09       & /                & /                & 35.10$\pm$0.09   & 54.04$\pm$0.08   & /                                    & /                                 \\ \hline
        AMQ      & 82.20$\pm$0.05        & 91.80$\pm$0.08       & /                & 66.49$\pm$0.12   & 55.26$\pm$0.13   & 67.83$\pm$0.08   & /                        & 69.65$\pm$0.14   \\ \hline
        AMQ-N    & 83.15$\pm$0.06        & 91.70$\pm$0.05       & /                & 66.66$\pm$0.12   & 55.50$\pm$0.06   & 67.70$\pm$0.03   & /                    & 70.01$\pm$0.12   \\ \hline
        ALQ      & 79.21$\pm$0.10        & 92.27$\pm$0.04       & /                & 67.35$\pm$0.09   & 45.74$\pm$0.07   & 69.10$\pm$0.10   & /                        & 70.87$\pm$0.10   \\ \hline
        ALQ-N    & 80.80$\pm$0.05        & 92.47$\pm$0.03       & /                & 66.78$\pm$0.12   & /                & 69.22$\pm$0.10   & /                                        & 70.83$\pm$0.06   \\ \hline
        CASQ      & \bfseries{92.49$\pm$0.04}        & \bfseries{92.88$\pm$0.05}       & \bfseries{66.57$\pm$0.11}   & \bfseries{67.47$\pm$0.06}   & \bfseries{68.86$\pm$0.05}   & \bfseries{69.24$\pm$0.04 }  & \bfseries{71.09$\pm$0.13 }  & \bfseries{71.29$\pm$0.10}   \\ \hline
    \end{tabular}
\end{table*}

==> section/cas_acc_proof.tex <==
\section{Theory analysis}


==> section/cas_implementation.tex <==

\section{Implementation of CAS-SGD}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{figures/framework}
	\caption[CAS-SGD Algorithm]{The CAS-SGD Algorithm}
	\label{fig:framework}
\end{figure}

In this section, we describe the implementation details of CAS-SGD based on the CAS quantization methodology. The process of SGD with CAS quantization is summarized in Algorithm~\ref{algo:sgdcas}. Our CAS-SGD framework is consist of four main procedures: Cluster analysis and sketch initialization at line~\ref{algo:clusterstart} to~\ref{algo:clusterend}; Quantization at line \ref{algo:quan_start} to \ref{algo:quan_end}; Gradients synchronization at line~\ref{algo:syncstart} to~\ref{algo:syncend}; Updating and error compensation at line~\ref{algo:dequan_start} to~\ref{algo:dequan_end}. Next, we list technologies used in these procedures, which boost the efficiency of the algorithm and mitigate the quantization loss with little extra overhead.



\IncMargin{1em}
\begin{algorithm}[t]
	\SetKwData{value}{Value}\SetKwData{counter}{Counter}\SetKwData{shape}{shape}
	\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}\SetKwFunction{Backpropagation}{Backpropagation}\SetKwFunction{AssignCluster}{AssignCluster}\SetKwFunction{InitCAS}{{InitCAS}}\SetKwFunction{Broadcast}{Broadcast}\SetKwFunction{Cluster}{Cluster}\SetKwFunction{Send}{Send}\SetKwFunction{ReduceCAS}{ReduceCAS}\SetKwFunction{Receive}{Receive}\SetKwFunction{Query}{Query}
	\SetKwFor{Paralleldo}{for}{do in parallel}{end}
	\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
	\SetKw{Continue}{continue}
	\SetKwInput{Initialization}{Initialization}
	\Input{$K$ - number of clusters; $ \tau $ - clustering interval; $ W $ - number of work nodes; $ X $ - input data}
	\Output{$\boldsymbol{\omega}_T$ - model parameters}
	
	\Initialization{ parameters $\boldsymbol{\omega}_0$, learning rate $ \eta_{0} $, error compensation $ e_0\leftarrow 0 $}
	\BlankLine
	\Paralleldo{$ i \leftarrow1 $ \KwTo $ W $}
	{
		\For{$t\leftarrow 1$ \KwTo $T$}
		{
			$g_t^i\leftarrow$ \Backpropagation{$\boldsymbol{\omega}_{t-1}, X^i_t$}\;
			%		\tcp{learn cluster centers every $ \tau  $ iterations}
			\If{t \% $\tau ==0$ } {\label{algo:clusterstart}$\mathbf{c}$ $\leftarrow$ \Cluster{$ g_t^i, K$}
			}		
			$  \tilde{{g}}_{t}^{i} \leftarrow \eta_{t}
			{g}_{t}^{i}+{e}_{t-1}^{i}  $\;
			%		 \tcp{Assign cluster for each gradient and return cluster assignment matrix}\label{algo:assign}
			$C^i \leftarrow $ \AssignCluster($g_t^i, \mathbf{c}$)\tikzmark{right}\;
			
			\If{t \% $\tau ==0$}
			{$S^i, A \leftarrow $ \InitCAS($ C^i, g_t^i $)\;
			}\label{algo:clusterend}
			%		\tcp{Initial sketch and set mapping matrix every $ \tau $ iterations}
			%		\Broadcast($S_t^i$.\shape $, \mathbf{c}$)\;
			\ForEach{cluster $k$}
			{	\label{algo:quan_start}
				$ \varLambda[k] \leftarrow diag(C^i[:, k])g_t^i $\;
				$Counter[k] \leftarrow diag({(A_k^TA_k)}^{-1})$\;
			}
			$ S^i  \leftarrow Counter \odot (A^T\varLambda) $\;
			%		\tcp{Average each bucket with element wise multiply}
			\label{algo:quan_end}
			\Send{$ S^i, C^i $}\label{algo:syncstart}\;
			$ S \leftarrow\frac{1}{W}\sum_{i=1}^{W}S^i $\tikzmark{top}\;\label{algo:adds}
			$ C \leftarrow \sum_{i=1}^{W}C^i $\;\label{algo:addc}
			%		$S, C \leftarrow$\ReduceCAS{${S}^1, C^1\dots, {S}^W, C^W$}\;
			\ForEach{cluster $k$}
			{	
				$\hat{g}_t[k] \leftarrow diag(C[:, k]) A S[k]$\;
			}
			$\hat{g}_t \leftarrow \frac{1}{W}\sum_{k=1}^{K}\hat{g}_t[k]$\tikzmark{bottom}\;
			
			%		\tcp{Query in Server}\label{algo:aggregate}
			\Receive($ \hat{g}_t  $)\label{algo:syncend}\;		
			$\boldsymbol{\omega}_t\leftarrow \boldsymbol{\omega}_{t-1}- \hat{g}_t $\label{algo:dequan_start}\;
			$ {e}_{t}^{i}=\tilde{{g}}_{t}^{i}-\hat{{g}}_{t} $ \label{algo:dequan_end}\;
			
			
		}
	}
	%	\SetKwProg{Def}{def}{:}{}
	%	\Def{ReduceCAS(${S}^1, C^1\dots, {S}^W, C^W$)}
	%	{
	%		$ S \leftarrow\frac{1}{W}\sum_{i=1}^{W}S^i $\;
	%		$ C \leftarrow \sum_{i=1}^{W}C^i $\;
	%		return $ S, C $\;
	%	}
	\AddNote{top}{bottom}{right}{Parameter Server}
	
	\caption{Cluster-Aware Sketch SGD}\label{algo:sgdcas}
\end{algorithm}\DecMargin{1em}


%gradient data pre-preparation and data structure
%cluster method: k-means in the sample; sync cluster center to keep theory and sync sketch shape to achieve linearity, $\tau$ ; assignment Pytorch implementation, positive and negative; especially for 1-bit quantization, further study multi-layer, each kind of layer is a cluster, partition them to positive and negative, can avoid assignment and sync; sketch initialization;
\subsection{Adaptive Clustering and Sketch Initialization}{\label{subsec:adaptive}}
After computing gradients with BP, we need to assign each gradient to its cluster. However, the cost of clustering on the whole gradients is prohibitive. We turn to sample the vector and learn the cluster centers as a model to assign total data. 

We implement the cluster assignment function based on \verb|Torch.Tensor|~\cite{paszke2019pytorch}, which can be accelerated in GPU. The assigned cluster center for a gradient is not only the nearest in distance but also the same sign, because the direction of optimization should be ensured. 

Then we adaptively initial the structure of the sketch with \verb|InitCAS|. Recall the inconsistent requirements of precision for distinct values of gradients, we set the number of buckets $ m $ based on the three characteristics of clusters: \emph{the number of gradients}, \emph{the magnitude of values} and \emph{{the entropy of a cluster}}. It is intuitive that the more gradients, the more buckets, and the bigger magnitude of values, the more precision of quantization. The higher entropy means that the values in a cluster are distributed evenly and require more buckets to distinguish them. 
%To enable acceleration on matrix operation with GPU, we set $ m $ for the cluster of the biggest magnitude as the shape of the sketch.

Note that the procedures \verb|Cluster| and \verb|InitCAS| are executed every $ \tau $ iterations in the implementation, because the gradients distributions among consecutive iterations are almost the same (as shown in Figure~\ref{fig:grad_distribution}(a)) and the efficiency of CAS-SGD can be improved with this setting. Function \verb|InitCAS| also maps each gradient to one of the $ m $ buckets with a random hash function. 

In Equation~\ref{eq:esti_grad_cluster} the algorithm quantize the gradients in each cluster with $(diag(C[:, k])A)^T(diag(C[:, k])g)$, we simplify this formula and merge them all into matrix to improve the time cost. Here we average each bucket with element-wise multiplication in the insertion procedure instead of the query phase to cut down half of the communication cost of the sketch.

%insert gradients and count  
%linearity of cas, reduce inverse comm
%\subsection{Efficient Quantization Encoding}
%The CAS method separate the gradients according to its empirical distribution, but not evenly part them like other quantization methods. Due to the density of the cluster with tiny gradients, we can encode them with 1-bit. In contrast, other quantization methods represent some tiny gradients with 2 or 3-bit. Thus, It provide an opportunity to reduce the communication cost by efficient encoding. In CAS-SGD, we implemented this with Huffman-Coding.

%In Equation~\ref{eq:esti_grad_cluster} the algorithm quantize the gradients in each cluster with $(diag(C[:, k])A)^T(diag(C[:, k])g)$, we simplify this formula and merge them all into matrix to improve the time cost. Here we average each bucket with element-wise multiplication in the insertion procedure instead of the query phase to cut down half of the communication cost of the sketch.

%query operation and error compesation
\subsection{ Mergeable CAS }

As other quantization methods do, we send the sketch $ S^i $ and compressed cluster assignment $ C^i $, the communication cost is $ O(N\log{K}) $. 

After collecting all the compressed data, the parameter server responsible for decompressing each gradients vector one by one and averaging them. However, as illustrated in the upper part of Figure~\ref{fig:merge}, it is time consuming in large scale distributed system. In practice, we merge these compressed data directly by element-wise addition at line~\ref{algo:adds} and~\ref{algo:addc}, then we have
\begin{align*}
	\sum_{i=1}^{W}{\sum_{k=1}^{K}{diag(C^i[:, k])AS^i[k]}}=&\sum_{k=1}^{K}{\sum_{i=1}^{W}{diag(C^i[:, k])AS^i[k]}}\\
	%	=&\sum_{k=1}^{K}{\left(\sum_{i=1}^{W}diag(C^i[:, k])\right)AS[k]}\\
	=&\sum_{k=1}^{K}{diag(C[:, k])AS[k]}
\end{align*}   

\begin{figure}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{figures/merge}
	\caption[Merge]{Synchronizing quantized gradients receiving from 16 nodes in PS, the top is querying one by one, the bottom is merging CAS before query operation.}
	\label{fig:merge}
\end{figure}

where we view $ S[k] $ as $ S^i[k] $ because the distribution of gradients among the worker nodes are almost the same (as illustrated in Figure~\ref{fig:grad_distribution}(b)). Then the query can be operated only once as shown in the bottom half of Figure~\ref{fig:merge}.

In particular, an further optimized method of query for 1-bit CAS quantization is transferring compressed $ C $ and $ S $ back to worker nodes and querying gradients by themselves. In this case, the download cost shrink to $ O(\log{W}/32) $ of the size of float gradients when the merged cluster assignment is encoded with $ N\log W $ bits.





==> section/preliminaries.tex <==
\section{Preliminaries}

We now formulate the gradients quantization methods based on stochastic projection and analyze the error of CM-based compression.


\subsection{Stochastic Projection Based Quantization Analysis}\label{subsec2.2}
Quantization method is one of the most popular methods to compress weights or gradients when train and deploy deep neural network, it maps the float data to several discrete buckets, which can be represented by much fewer bits. A lot of researches exploit quantization to reduce communication cost by compressing gradients in distributed DL training. Let ${g, \hat{g}}\in {\mathbb{R}^d}$ denote the vector of gradients computed in BP and estimated in de-quantization operation respectively, and $\bar{g}$ denote that on whole dataset. Let $m, N$ denote the number of buckets and gradients being quantized respectively. Let $A \in \{0, 1\}^{N \times m}$ denote the indicator matrix, and $A(i, j) = 1$ iff the $i^{th}$ item ${g}_i$ is mapped to the $j^{th}$ bucket, where $j\in [1,m]$, otherwise $A(i,j)=0$. Any quantization method can be represented with this stochastic projection: $\hat{g}=Af(g)$. We formulate the objective of gradients quantization as formula \ref{eq2:quant_obj}:

\begin{equation}\label{eq2:quant_obj}
	\min _{A}\left\|{g}-A f(g)\right\|_{2}^{2}	
\end{equation}  

For example, two widely used quantization schemes, QSGD~\cite{alistarh2017qsgd} and TernGrad~\cite{wen2017terngrad}, both can be fitted into the projection.  When the number of quantization buckets $m=2$, they decide which buckets should be mapped to for $g_i$ according to $sign(g_i)\zeta_{i}$, where $\zeta_{i}\sim Bernoulli(|{|g_i|}|/ \|g\|_q)$, $q=2$ for QSGD and $\infty$ for TernGrad, while $f(g)$ outputs the vector of ${ [-\|g\|_q,  \|g\|_q ]^T}$. 

\subsection{Stochastic Projection Based Sketch Compression Analysis}
Sketch is a data flow statistics estimation technology that inserts the data value into a sketch data structure and returns an approximate value over bucket arrays in the query phase. Count-Min Sketch (CM) \cite{cormode2005improved} is the most popular sketch method, it adds one value to several bucket arrays, one bucket each array, which chosen by a specific uniformly-random hash function, and returns the minimum value of those mapped buckets as the estimation value. 

Assumed that a sketch structure consists of one bucket array, the gradients compression with count-min sketch can also be fitted into stochastic projection:  The insertion operation is equivalent to $A^T g$, where $A$ is defined as that in Section. \ref{subsec2.2}, and the query phase corresponds to $\hat{g}=AA^{T}g$. 

Let $\mu$ and $\sigma{^2}$ denote the expectation and variance of a gradient upon stochastic gradients $g$ respectively. Here we analysis the expectation and variance of the loss of CM compression from stochastic projection perspective following the work in \cite{fu2020clustering}: 

\begin{theorem}\label{theo:cmloss}
	Suppose that each entry in $g$ is independent and identically distributed (i.i.d.) with expectation $\mu$ and variance $\sigma{^2}$. The expectation of the loss of each entry $j\in[1, N]$ respect to ${g}(j)$ is $\frac{(N-1) \mu}{m}$ and the variance is $\frac{N-1}{m}\left(\sigma^{2}+\left(1-\frac{1}{m}\right) \mu^{2}\right)$
	
\end{theorem}

\begin{iproof}[Proof Sketch]\label{proof:cmloss}
	The loss of a sketch can be quantified as $\hat{g}-g=A A^{T} g-g=\left(A A^{T}-I\right) g$, where $I$ denotes the identity matrix. $AA^T$ is a $N\times N$ symmetric matrix, where each entry $(i, j)$ is one when the $i^{th}$ and $j^{th}$ gradients mapped into the same bucket, {i.e.}: $A(i, :)=A(j, :)$, and zero otherwise. It means that the diagonal entries are all set to ones.  Each gradients is mapped according to a uniformly-random hash function, so that $Pr[AA^T(i, j)=1]=\frac{1}{m}$ and $Pr[AA^T(i, j)=1]=1-\frac{1}{m}$, which follows Bernoulli distribution. 
	
	Let $\Phi=AA^T-I$, then each non-diagonal entry in $\Phi$ is the same as that in $AA^T$,  we have $\Phi_{i\neq j}(i, j)\sim Bernoulli(\frac{1}{m})$, and the diagonal entries are zeros, which means $\mathbb{E}[\Phi_{i\neq j}(i, j)]=\frac{1}{m}$ and $Var[\Phi_{i\neq j}(i, j)]=\frac{1}{m}\cdot(1-\frac{1}{m})]$
	
	We can deduce the expectation of estimation loss respect to ${g}(j)$ as shown in Appendix~\ref{appen:cmloss} 
\end{iproof}
Based on the Theorem~\ref{theo:cmloss}, the queried value from count-min sketch is not the unbiased estimation of $\bar{g}$, and its variance of loss is proportional to the average number of elements in each bucket, which impede the convergence of distributed SGD. We proposed Cluster-Aware-Sketch quantization to address these issues.











==> section/related_works.tex <==
\section{Related Work}
%\vspace{1mm}\noindent\textbf{Communication Efficient Distributed Training}
\vspace{1mm}\noindent\textbf{Communication Efficient Distributed Training}
%The natures of stochastic gradients in deep learning allow applying lossy compression such as quantizing or sparsifying the gradients. 
The scalability of distributed deep learning system is limited by the gradient synchronization time~\cite{you2017scaling}, and many recent communication efficient systems have been proposed to overlap the cost~\cite{abadi2016tensorflow, zhang2017poseidon,li2018pipe,huang2018gpipe,  shi2019mg, narayanan2019pipedream, rasley2020deepspeed, fan2021dapple}. On the other hand, gradient compression algorithms also draw researcher's attention to reduce the communication traffic. The current gradient compression method can be categorized into three types, quantization, sparsification and low-rank approximation.
Quantization is a widely used gradient compression method because of its solid convergence guarantee~\cite{alistarh2017qsgd,wen2017terngrad,bernstein2018signsgd,karimireddy2019error}. The remarkable studies on quantization, such as QSGD~\cite{alistarh2017qsgd} normalize and quantize each gradient with a set of uniform quantization levels, then represent the gradients with fewer bits. TernGrad~\cite{wen2017terngrad} is a special case of QSGD, which only have three quantization levels. 
Besides, another line of compression methods aggressively sparsify the gradient and only send those significant~\cite{stich2018sparsified,lin2018deep,wangni2018gradient,renggli2019sparcml, shi2019convergence,chen2020scalecom}. Also, Some recent works use Singular Value Decomposition to compress the gradient~\cite{yu2018gradiveq, wang2018atomo, vogels2019powersgd}, which enable the linear computation on the compressed gradient. In this paper, we focus on the quantization method.

%CASQ method is equivalent to sparsification when only allocating one bucket array and mapping those significant gradients into the buckets. In this paper, we focus on compression error minimization in a general setting and leave the study of applying CAS to sparsification as future work.  

%These methods yield unbiased estimation of stochastic gradients to maintain the convergence of SGD. Meanwhile, some biased sign-based quantization~\cite{karimireddy2019error} have competent convergence when using error-feedback technology proposed in~\cite{stich2018sparsified}.
\vspace{1mm}\noindent\textbf{Adaptive Quantization}
Some prior attempts pay attention to the quantization of the non-uniform distributed gradients. ZipML~\cite{zhang2017zipml} dynamically finds the optimal quantization levels, but it is difficult to quantize gradients on the fly. NUQSGD~\cite{ramezani2019nuqsgd} and Natural Compression (NC)~\cite{horvath2019natural} quantize gradient with exponentially spaced levels. TINYSCRIPT~\cite{fu2020don} finds the quantization levels with minimum variance based on modelling gradients with Weibull distribution. Faghri et al.~\cite{faghri2020adaptive} proposed ALQ and AMQ. ALQ minimizes the variance of quantization by computing the optimal levels on the estimated gradient distribution. AMQ models the quantization levels as exponentially spaced levels and solves for the optimal multiplier of the levels. However, the variance reduction of these adaptive methods is limited by the discrete quantization levels. 

\vspace{1mm}\noindent\textbf{Sketch-based Gradient Compression}
% These sparsification methods also apply error-feedback to accumulate and postpone the updates. 
Sketch-based methods are introduced in large-scale training by Sketch-SGD~\cite{ivkin2019communication} and in federated learning by FetchSGD~\cite{rothchild2020fetchsgd}. However, the errors of these methods are bounded with $ {L}^2 $ norm. Thus they can only approximate the Top-K gradients. Prior study~\cite{jiang2020skcompress} uses quantile sketch and Min-Max sketch to approximate the quantiles of gradient, but it focuses on linear models and is ill-suited to GPU-based deep learning system.
%We also design CAS-SGD for GPU based distributed deep learning system and prove the convergence of our method.

%Prior works of cluster-based~\cite{han2015deep} and sketch based~\cite{spring2019compressing} quantization methods compress the weights such as convolution kernels to employ the model in edge devices. They focus on the performance of model inference while we address the communication cost in distributed model training.
%\vspace{1mm}\noindent\textbf{Compressed Gradient Aggregation}
%Efficient aggregation is also crucial for high scalability, \cite{yu2018gradiveq,vogels2019powersgd} compute a low-rank approximation of gradient, and achieve scalability in ring all-reduce system by linear compressor operators. They rely on, however, the gradients decomposition, which usually cannot compress the vector when combining gradients from several layers to communicate. The sketch-based works~\cite{ivkin2019communication} address this issue, and we also implement the linearity in our CAS method.

